The Complexity of Games with Randomised Control

We study the complexity of solving two-player infinite duration games played on a fixed finite graph, where the control of a node is not predetermined but rather assigned randomly. In classic random-turn games, control of each node is assigned randomly every time the node is visited during a play. In this work, we study two natural variants of this where control of each node is assigned only once: (i) control is assigned randomly during a play when a node is visited for the first time and does not change for the rest of the play and (ii) control is assigned a priori before the game starts for every node by independent coin tosses and then the game is played. We investigate the complexity of computing the winning probability with three kinds of objectives-reachability, parity, and energy. We show that the qualitative questions on all variants and all objectives are NL-complete. For the quantitative questions, we show that deciding whether the maximiser can win with probability at least a given threshold for every objective is PSPACE-complete under the first mechanism, and that computing the exact winning probability for every objective is sharp-P-complete under the second. To complement our hardness results for the second mechanism, we propose randomised approximation schemes that efficiently estimate the winning probability for all three objectives, assuming a bounded number of parity colours and unary-encoded weights for energy objectives, and we empirically demonstrate their fast convergence.

==> fig-explicit-whole.tex <==
%!TEX root = ./main.tex

\scalebox{.7}{
\begin{tikzpicture}[scale=1, >=latex', shorten >=2pt, node distance=.7cm and 1.2cm, on grid, auto]

    %Level 0
    %Graph epsilon
    \node[state] (n1) {$v_0$};
    \node[state, above right=of n1] (n2) {$v_1$};
    \node[state, below right=of n1] (n3) {$v_2$};
    \node[state, right=2.4cm of n1] (n4) {$\top$};

    
    \path[->] (n1) edge[bend left] (n2);
    \path[->] (n2) edge[bend left] (n1);
    \path[->] (n1) edge[bend left] (n3);
    \path[->] (n3) edge[bend left] (n1);
    \path[->] (n2) edge (n4);
    \path[->] (n3) edge (n4);
    \path[->] (n4) edge[loop above] (n4);

    %Level 1

    %Graph 0
    \node[state, below left =2.7cm and 3cm of n3, fill=blue!20] (0n1) {$v_0$};
    \node[state, above right=of 0n1] (0n2) {$v_1$};
    \node[state, below right=of 0n1] (0n3) {$v_2$};
    \node[state, right=2.4cm of 0n1] (0n4) {$\top$};

    \path[->] (0n1) edge[bend left] (0n2);
    \path[->] (0n2) edge[bend left] (0n1);
    \path[->] (0n1) edge[bend left] (0n3);
    \path[->] (0n3) edge[bend left] (0n1);
    \path[->] (0n2) edge (0n4);
    \path[->] (0n3) edge (0n4);
    \path[->] (0n4) edge[loop above] (0n4);

   % Graph 1
    \node[state, below right =2.7cm and 1cm of n3, pattern=grid, pattern color=red!50] (1n1) {$v_0$};
    \node[state, above right=of 1n1] (1n2) {$v_1$};
    \node[state, below right=of 1n1] (1n3) {$v_2$};
    \node[state, right=2.4cm of 1n1] (1n4) {$\top$};

    \path[->] (1n1) edge[bend left] (1n2);
    \path[->] (1n2) edge[bend left] (1n1);
    \path[->] (1n1) edge[bend left] (1n3);
    \path[->] (1n3) edge[bend left] (1n1);
    \path[->] (1n2) edge (1n4);
    \path[->] (1n3) edge (1n4);
    \path[->] (1n4) edge[loop above] (1n4);

    % Level 2

    %Graph 00

    \node[state, below left =2.7cm and 3cm of 0n3, fill=blue!20] (00n1) {$v_0$};
    \node[state, above right=of 00n1] (00n2) {$v_1$};
    \node[state, below right=of 00n1] (00n3) {$v_2$};
    \node[state, right=2.4cm of 00n1] (00n4) {$\top$};

    \path[->] (00n1) edge[bend left] (00n2);
    \path[->] (00n2) edge[bend left] (00n1);
    \path[->] (00n1) edge[bend left] (00n3);
    \path[->] (00n3) edge[bend left] (00n1);
    \path[->] (00n2) edge (00n4);
    \path[->] (00n3) edge (00n4);
    \path[->] (00n4) edge[loop above] (00n4);

    %Graph 10
    \node[state, below left =2.7cm and 3cm of 1n3, fill=blue!20] (10n1) {$v_0$};
    \node[state, above right=of 10n1] (10n2) {$v_1$};
    \node[state, below right=of 10n1] (10n3) {$v_2$};
    \node[state, right=2.4cm of 10n1] (10n4) {$\top$};

    \path[->] (10n1) edge[bend left] (10n2);
    \path[->] (10n2) edge[bend left] (10n1);
    \path[->] (10n1) edge[bend left] (10n3);
    \path[->] (10n3) edge[bend left] (10n1);
    \path[->] (10n2) edge (10n4);
    \path[->] (10n3) edge (10n4);
    \path[->] (10n4) edge[loop above] (10n4);

    % Rectangles
    \node[draw, rounded corners, thick, fit=(n1)(n2)(n3)(n4),] (boxTop) {};
    \node[draw, rounded corners, thick, fit=(0n1)(0n2)(0n3)(0n4),] (boxLeft) {};
    \node[draw, rounded corners, thick, fit=(1n1)(1n2)(1n3)(1n4),](boxRight) {};
    \node[draw, rounded corners, thick, fit=(00n1)(00n2)(00n3)(00n4),] (boxLeftLeft) {};
    \node[draw, rounded corners, thick, fit=(10n1)(10n2)(10n3)(10n4),] (boxRightLeft) {};
    %Empty nodes
    \node[below left=2cm and 1cm of boxLeft] (voidA) {};
    \node[below right=2cm and 1cm of boxLeft] (voidB) {};
    \node[below left=2cm and 1cm of boxRight] (voidC) {};
    \node[below right=2cm and 1cm of boxRight] (voidD) {};

    %Edges between rectangles

    \draw[->, very thick] (boxTop.south) -- node[midway, left=5mm, font=\small]{$\frac{1}{2}$} (boxLeft.north);
    \draw[->, very thick] (boxTop.south) -- node[midway, right=5mm, font=\small]{$\frac{1}{2}$} (boxRight.north);
    
    \draw[->, very thick] (boxLeft.south) -- node[midway, left=2mm, font=\small]{$v_1$} (voidA);
    \draw[->, very thick] (boxLeft.south) -- node[midway, right=2mm, font=\small]{$v_2$} (voidB);

    \draw[->, very thick] (boxRight.south) -- node[midway, left=2mm, font=\small]{$v_1$} (voidC);
    \draw[->, very thick] (boxRight.south) -- node[midway, right=2mm, font=\small]{$v_2$} (voidD);
\end{tikzpicture}
}

==> fig-explicit.tex <==
%!TEX root = ./main.tex


\begin{tikzpicture}[scale=0.5, >=latex', shorten >=1pt, node distance=.7cm and 1.2cm, on grid, auto]
    % Nodes
    \node[state] (n1) {$v_0$};
    \node[state, above right=of n1] (n2) {$v_1$};
    \node[state, below right=of n1] (n3) {$v_2$};
    \node[state, right=2.4cm of n1] (n4) {$\top$};

    \node[state, below left =4cm of n3,fill=blue!20] (0n1) {$v_0$};
    \node[state, above right=of 0n1] (0n2) {$v_1$};
    \node[state, below right=of 0n1] (0n3) {$v_2$};
    \node[state, right=2.4cm of 0n1] (0n4) {$\top$};

    \node[state, below right =4cm of n3,pattern=grid, pattern color=red!50,] (1n1) {$v_0$};
    \node[state, above right=of 1n1] (1n2) {$v_1$};
    \node[state, below right=of 1n1] (1n3) {$v_2$};
    \node[state, right=2.4cm of 1n1] (1n4) {$\top$};

    

    \path[->] (n1) edge[bend left] (n2);
    \path[->] (n2) edge[bend left] (n1);
    \path[->] (n1) edge[bend left] (n3);
    \path[->] (n3) edge[bend left] (n1);
    \path[->] (n2) edge (n4);
    \path[->] (n3) edge (n4);
    \path[->] (n4) edge[loop right] (n4);

    \path[->] (0n1) edge[bend left] (0n2);
    \path[->] (0n2) edge[bend left] (0n1);
    \path[->] (0n1) edge[bend left] (0n3);
    \path[->] (0n3) edge[bend left] (0n1);
    \path[->] (0n2) edge (0n4);
    \path[->] (0n3) edge (0n4);
    \path[->] (0n4) edge[loop right] (0n4);

    \path[->] (1n1) edge[bend left] (1n2);
    \path[->] (1n2) edge[bend left] (1n1);
    \path[->] (1n1) edge[bend left] (1n3);
    \path[->] (1n3) edge[bend left] (1n1);
    \path[->] (1n2) edge (1n4);
    \path[->] (1n3) edge (1n4);
    \path[->] (1n4) edge[loop right] (1n4);

\end{tikzpicture}


==> fig-reach-exmp.tex <==
%!TEX root = ./main.tex


\begin{tikzpicture}[scale=0.8, >=latex', shorten >=1pt, node distance=1cm and 1.2cm, on grid, auto]
    % Nodes
    \node[state, initial, initial text=] (n1) {$v_0$};
    \node[state, above right=of n1] (n2) {$v_1$};
    \node[state, below right=of n1] (n3) {$v_2$};
    \node[state, right=2.7cm of n1] (n4) {$\top$};

    \path[->] (n1) edge[bend left] (n2);
    \path[->] (n2) edge[bend left] (n1);
    \path[->] (n1) edge[bend left] (n3);
    \path[->] (n3) edge[bend left] (n1);
    \path[->] (n2) edge (n4);
    \path[->] (n3) edge (n4);
    \path[->] (n4) edge[loop above] (n4);
\end{tikzpicture}


==> rebuttal.tex <==
Thank you for taking the time to review our paper. We appreciate your positive comments. We will implement all editorial feedback in the revision and focus here on the raised questions.

Review 1

"complexity of almost-sure winning of standard random-turn games with parity and energy objectives"

Our main reason for covering Theorems 2 and 3 is that they are needed for Theorem 4, which is important because previously the question "is there a simple translation from stochastic games to random-turn games?" was open, and we found it insightful that, if we want it to be probability preserving, this would entail NL=P.

For this purpose, the current version of Theorem 2 is good enough.

We leave the extension to parity and energy as future work. It is at least not straightforward, as these games retain aspects of a two-player game, while "surely" (Theorem 3) creates a one-player game where Min makes all decisions.

Review 3

"motivation of the proposed games with random control"

Formal verification and synthesis are mentioned at the beginning as motivations for studying general two-player graph games. Dynamic control of nodes has already been studied for games in verification (see Related works). Random-turn games have also been studied and proved to be equivalent to a variant of another well studied dynamic control game in verification-- bidding games [23] (ln 128). Our variations of games with random control arise as natural variations of random-turn games. These variants exactly capture scenarios where ownership of a node is a function of a single random event. Our proposed games also have potential applications in system design, where winning probabilities can serve as a measure of fairness (ln 593–599).

Once defined, studying these games seems natural, and we still think that studying natural variations of two-player games on graph with clean complexity results falls well within the scope of FoSSaCS.

"why counting problem for random arena" 

The value in random-arena variant closely connected to the proportion of winning games, which is naturally a counting problem.

Review 4

"the novelty of almost-sure and sure winning in standard random-turn games"

As far as we know, the results for almost-sure and sure winning in standard random-turn games do not appear in the literature. Since they are not hard to obtain, we do not present them as our main contributions. we claim as our contributions only the complexity results (NL-complete) for the qualitative problems for our two variants of games.

"games with random control vs. general stochastic games"

In ordinary stochastic games, both players have positional optimal strategies, whereas unfolding random-turn games and random arena games, the optimal strategy depends on the partial unfolding seen so far and the initial allocation of control. This adds complexity for the quantitative case.

For the qualitative case, the situation is quite different: we have to consider only the case where one player wins all the (finitely many) coin tosses, so all that remains is a non-stochastic one-player game.

"unified view of unfolding random-turn games and random-arena games"

One way to look at unfolding random-turn games is to view them as random arena games with incomplete information, where the arena is fixed, but the players do not initially know the randomly selected arena. In that view, the probability distribution over arenas is the same.

Incomplete information does not a priori favour a particular player in that case, as both players would have the same information: namely, the allocation of the vertices visited.

When taking this view, one *could* play with variations, such as making one player's information on the allocation complete while keeping the other player's view partial.

------------------------------------------------------
------------------------------------------------------

Thank you all for taking the time to review our paper. We appreciate your positive comments. We will implement the editorial feedback in the revision and focus below on the raised questions.

Review 1

"complexity of almost-sure winning of standard random-turn games with parity and energy objectives"

Our main reason for covering Theorems 2 and 3 are that they are needed for Theorem 4, which is important because previously the question "is there a simple translation from stochastic games to random-turn games?" was open, and we found it insightful that, if we want it to be probability preserving, this would entail NL=P.

For this purpose, the current version of Theorem 2 is good enough.

We leave the extension to parity and energy as future work. It is at least not straightforward, as these games retain aspects of a two-player game, while surely (Theorem 3) creates a one-player game where player Min makes all decisions.


"restrictions should appear in the abstract"
Thank you. We will make it explicit in the abstract.

Review 3

"motivation of the proposed games with random control"

Formal verification and synthesis are mentioned at the beginning as motivations for studying general two-player graph games. Dynamic control of nodes has already been studied for games in verification (see Related works). (Standard) random turn games have also been studied and proved to be equivalent to a variant of another well studied dynamic control game-- bidding games[23](ln 128).  Our variations of games with random control arise as natural variations of (standard) random-turn games. These variations are relevant in scenarios where ownership of a node is a function of a single random event. Our proposed games also have potential applications in game design, where winning probabilities can serve as a measure of fairness (lines 593–599).

Once defined, studying these games seems natural, and we still think that studying natural variations of two-player games on graph with clean complexity results falls squarely into the scope of FoSSaCS.

"value problem for unfolding vs counting problem for random arena" "value problem for random-turn game"
The value in random arena game is given by the number of winning arenas, which is naturally a counting problem. Value problem for random-turn games are in NP \cap co-NP with reduction to stochastic games(Ln 65). 

"l.180, "winning" is not defined"
Winning is defined in the same subsection for respective games (line 169, line 172, line 178). We will make the winning probabilities in random games explicit after line 200. 

"energy games..NL(l.240)"
The NL algorithm guesses the entry point of the lasso. 2 counters are needed for the energy, one for total, one for sum in lasso. 

Review 4

"the novelty of almost-sure and sure winning in standard random-turn games"

As far as we know, the results for almost-sure and sure winning in standard random-turn games do not appear in the literature. Since they are not hard to obtain, we do not present them as our main contributions. we claim as our contributions only the complexity results (NL-complete) for the qualitative problems for our two variants of games.

"games with random control vs. general stochastic games"

In ordinary stochastic games, both players have positional optimal strategies, whereas unfolding random-turn games and random arena games, the optimal strategy depends on the partial unfolding seen so far and the initial allocation of control. This adds complexity for the quantitative case.

For the qualitative case, the situation is quite different: we have to consider only the case where one player wins all the (finitely many) coin tosses, so all that remains is a non-stochastic one-player game.

"unified view of unfolding random-turn games and random arena games"

One way to look at unfolding random-turn games is to view them as random arena games with incomplete information, where the arena is fixed, but the players do not initially know the randomly selected arena. In that view, the probability distribution over arenas is the same.

Incomplete information does not a priori favour a particular player in that case, as both players would have the same information, namely the allocation of the vertices visited.

When taking this view, one *could* play with variations, like making the information of one player on the allocation complete while keeping the other player's view partial.


------------------------------------------------------
------------------------------------------------------
(600 words limit)
Questions and ideas below
------------------------------------------------------
------------------------------------------------------

Review 1

Questions for rebuttal:

1. If I didn't miss anything then there are no result for almost sure winning of random turn games with parity and energy. Can you comment on that case?

(Rasmus: We might not want to write this, because this is not in the paper, but: Parity games should be NL complete too for almost sure winning and random turn games: You can win almost surely unless your oppoent can win with positive probability. Winning with positive pr. consists of finding a reachable state v from the initial state, and a parity p that is winning for you so that for all states reachable from v, a state of parity p is reachable - in each case, reachable is in the sense of one player reachable. This is all in NL. The condition is trivially sufficient - just go to v (which requires at most n steps and thus you can do so with positive probability, by winning the first n times) and you are then almost sure winning, since you can always get p by just winning the coin flip at most n times in a row. It is necessary since as long as as the maximum parity can be restricted more, one player might as well do it. More precisely, assume that no such state v exists: The probability of winning is then 0, because the following strategy is almost sure winning for the other player. At each point in time, the other player will move towards a reachable state v' so that the maximum parity p' reachable from v' is as small as possible or, if the maximum parity is already as restricted as possible, move towards a state of parity p'. v' does not satisfy the definition of v, hence p' is winning for the other player and v' is thus almost sure winning for the other player, since they can get to v' and get p' by being lucky at most n times in a row).


2. In the abstract and the introduction you mention that computing the values of random arena games can be approximated and one can easily get the impression that this holds for all three winning conditions, but it turns out that one needs restrictions to obtain the upper bound for parity (few colors) and energy (unary encoding of weights). I would say these restrictions should appear in the abstract and introduction.

------------------------------------------------------

Review 2

- what about mixing parity and energy objectives ? Do you need further investigations
or the results in the paper are able to handle this combination?
-l108. As far as I can judge, safety is not explicitly handled in the paper, but can
be obviously captured with parity.
-l509. Is [21] really the right reference for the upper bound UP \cap co-UP for
energy games?
-l549. As far as I understand, this would work for any restriction that leads to
polynomial-time solvability. Is it correct ?

------------------------------------------------------

Review 3

The main drawback of the paper is the lack of motivation. The paper refers
to formal verification and synthesis, but gives no hint of how their model
could be used in that context, where typically inputs are chosen by one
player (the environment), and outputs are chosen the other player (the system).
For example, how would it make sense that inputs are sometimes chosen by the
system, and outputs by the environment?
------------------------------------------------------

Review 4

– Regarding the NL upper bound for almost-sure and sure winning in standard random-turn games:
The paper presents a fresh NL-membership argument. However, since random-turn qualitative reachability reduces directly to directed reachability (ST-CONNECTIVITY), which is NL-complete, the upper bound appears to follow from standard reductions.
Could the authors clarify whether their upper-bound argument is intended as a novel contribution, or whether it simply re-derives a known result? If the latter, it may help to cite the standard NL upper bound (via ST-CONN) to avoid suggesting unintended novelty.



- The paper shows that deciding almost-surely winning or surely winning in games with randomised control (random-turn, unfolding random-turn, and random arena) admits a better upper bound than corresponding qualitative problems in general stochastic games.
On the other hand, deciding or computing the exact winning probability in unfolding random-turn or random arena game appears to admits a worse upper bound than the quantitative value problems in general stochastic games.
Could the author(s) elaborate on why this "flip" in complexity occurs? Is it inherent to the role of randomness in these models (hence, standard, and can be seen in other places as well) or is it accidental? A paragraph addressing this point might improve the conceptual clarity of the paper.

Overall it seems somewhat "accidental": That sure and almost sure coincides for unfolding random-turn and random arena games comes from them using a finite amount of randomness. Hence, intuitively, random-turn games are harder than the other classes for almost sure, since that does not coincide with sure. Conversely, unfolding random-turn games feels initutively harder than random arena games which in turn in general are about counting how many underlying deterministic games are winning. Counting releates to #P. Random-turn games are easier than turn-based stochastic games which is somewhat below NP. #P is harder than NP. 


 
- In the qualitative setting, the paper nicely connects the three randomised-control models (standard random-turn, unfolding random-turn, and random-arena games). For the quantitative questions, however, the complexity behaviour appears to diverge across the models. Could the authors comment on whether similar conceptual connections exist on the quantitative side, or explain why such a unifying view might be difficult?
One possible interpretation is that a random-arena game represents a probability distribution over all arenas compatible with a game graph, while an unfolding random-arena game represents only a subset of them (some vertices may never be assigned ownership on some paths in the explicit game). If this perspective is meaningful, could it give hints toward a more general or unified theory of randomised control (which may include the standard random-turn model, and open up the need or the lack thereof for new models with randomised control)?

